A survey for variable young stars with small telescopes: VII -- Spot Properties on YSOs in IC5070

We present measurements of spot properties on 31 young stellar objects, based on multi-band data from the HOYS (Hunting Outbursting Young Stars) project. On average the analysis for each object is based on 270 data points during 80 days in at least 3 bands. All the young low-mass stars in our sample show periodic photometric variations. We determine spot temperatures and coverage by comparing the measured photometric amplitudes in optical bands with simulated amplitudes based on atmosphere models, including a complete error propagation. 21 objects in our sample feature cool spots, with spot temperatures 500 - 2500 K below the stellar effective temperature ($T_{\rm eff}$), and a coverage of 0.05 - 0.4. Six more have hot spots, with temperatures up to 3000 K above $T_{\rm eff}$ and coverage below 0.15. The remaining four stars have ambiguous solutions or are AA Tau-type contaminants. All of the stars with large spots (i.e. high coverage $>0.1$) are relatively cool with $T_{\rm eff} < 4500$ K, which could be a result of having deeper convection zones. Apart from that, spot properties show no significant trends with rotation period, infrared excess, or stellar properties. Most notably, we find hot spots in stars that do not show $K-W2$ infrared excess, indicating the possibility of accretion across an inner disk cavity or the presence of plage.

==> 2nd_reply.tex <==
>>> We have carefully considered the comments by the referee and have revised our paper accordingly.  All changes made to the paper are typeset in bold-face. Please see below for the detailed replies to the referees comments. Our replies are marked with a '>>>'.

Dear Authors,
I have carefully read the revised version of the manuscript "A survey for variable young stars with small telescopes: VII - Spot Properties on YSOs in IC 5070" by Herbert et al.. I acknowledge that an effort was made in the revised version to show what is new in methodology and results that deserve publication in MNRAS. The authors analyze 31 young stellar objects with periodic multi-band light curves and obtain the spot temperatures and coverage by comparing observed and theoretical photometric amplitudes. The results agree with others in the literature and add a few more stars with well determined spot temperatures.

I have only two comments on the added material that I list below.

*Abstract, last paragraph:
The discussion about the presence of hot spots in stars that do not present IR excess in Sect. 4.3 is quite nice now and this last sentence of the abstract does not reflect the conclusion that the lack of K-W2 excess does not exclude the presence of a disk with an inner cavity or accretion. In Sect. 4.3 you also discuss the possibility that the hot spots could be due to plages. In the abstract, it is simply highlighted that hot spots can be present without an inner disk, which may lead the reader to a wrong conclusion.
>>> Reply: We have changed the final sentence of the abstract to better reflect our discussion, we also have edited the second-to-last paragraph of our conclusion to ensure consistency.

*Introduction, 1st paragraph, a suggestion of text:
...Hot spots are only expected to appear on accreting stars (classical T Tauri stars), that have either full or transition disks (Class II objects).
>>> Reply: We have included this text in the introduction as requested.

==> reply.tex <==
>>> We have carefully considered the comments by the referee and have revised our paper accordingly. We have clarified more clearly how our methodology is an improvement over previous works to address the main comment by referee. We also note that several of the comments are caused by a miss-understanding of our notation and have clarified accordingly. We agree with the points made about the temperature contrast between hot spots and YSO surface and have revised these sections. All changes made to the paper are typeset in bold-face. Please see below for the detailed replies to the referees comments. Our replies are marked with a '>>>'.

I have carefully read the manuscript "A survey for variable young stars with small telescopes: VII - Spot Properties on YSOs in IC 5070" by Herbert et al. It is well written, but it is not clear what are the new results that deserve to be published in MNRAS.  The authors analyze 31 young stellar objects with periodic multi-band light curves and obtain the spot temperature and coverage by comparing observed and theoretical photometric amplitudes. Their results agree with others in the literature. This type of work was, however, extensively done since the early 90's in projects such as COYOTES (Bouvier et al. 1993, 1995 etc), as acknowledged in the present manuscript. I would strongly advise, in the case of re-submission, to highlight the contribution of this work to what is already established about spot properties of young stars in the literature.

>>>Reply: We agree that our method is based on previous works going back to early 90's. However, as was outlined in the paper draft, to the best of our knowledge no-one has performed such an analysis by simultaneously considering multi-filter optical light curves, using stellar template spectra, and fully treating all aspects of the uncertainties of the methodology, including the identification of non-spot sources. Furthermore, no-one has so far measured the spot properties for any objects in the IC5070 star forming region, and this work forms the basis to study the evolution of these and other spotted objects over time. We have made some adjustments of the text in the introduction to clarify these points. Fitting optical multi-filter light curves to gain information on spots has actually not been used in a lot in the literature on YSOs, as most monitoring is done in one band. We would argue that building upon a method that is well-established, and applying that method to an entirely new sample of stars, is a valid contribution to the field. Finally, our extensive literature search has shown that there is no literature on links between spot properties and disks, rotation, and stellar parameters. 

I have several comments to help improve the manuscript, that I list below.

*Introduction, 3rd paragraph: Please explain how the spot temperature and coverage allow to verify and check models of magnetic field structure and generation in young stars.

>>>Reply: We have removed this statement from the introduction.

*Introduction, 4th paragraph: The aim of the manuscript is to establish a method that reliably recovers the properties of spots in YSOs from broadband photometry. This is already well established since more than 30 years, as shown in a series of papers by the COYOTES collaboration, for example. It is not clear that the proposed method, which is quite similar to others available, add something new to the analysis of variability amplitude to recover spot properties in the literature.

>>>Reply: Please see our reply to the main comment at the beginning of this response.

*Figure 1: The caption says V-I vs V but the vertical axis label indicates "I" magnitudes.

>>> Reply: Thank you. This typo has been fixed.

*Sect. 2.2, 3rd paragraph: The last sentence says that the two brighter objects have no measured Teff. Actually, in Fig. 1 there are 5 objects without literature Teff, which had their Teff estimated in the present work.

>>> Reply: Six objects have no literature Teff, and two of these are the brighter objects. In order to clarify this, we have rephrased how we present the information in this section. Information about colours that was previously in Sect. 2.3 has now been worked in to Sect. 2.2 to make it more clear. 

*Sect. 2.3, 2nd paragraph: Please give a reference to the relation Teff vs V-I used
to estimate the effective temperature of the two brightest objects in Fig. 1.

>>> Reply:  The Teff was assumed based on the V-I colours for the objects with known Teff, rather than from a relation in the literature. In reworking this into Sec. 2.2, we hope this is more clear now.

*Sect. 3.1, 1st paragraph: What is the effect on the spot temperature of not
considering limb darkening in your models? You cite the work of Bouvier et al. (1995)
but they actually consider a star with limb darkening.

>>>Reply: Including limb darkening will have a tiny effect on the spot size and an even smaller effect on the spot temperatures. In both cases these are significantly smaller than the statistical uncertainties of the method. We have included a paragraph with a description to reassure the reader of the legitimacy of our approach. Limb darkening will have a much stronger effect on the light curves, which we do not model in this work.

*Sect. 3.1, 1st paragraph: It would be important to show the light curves in an appendix, or at least one example of a cold spot, a hot spot and a dipper (AA Tau) light curve.

>>> Reply: All the light curves investigated here have already been published in this series. In particular all the IC5070 phase folded light curves are in Froebrich et al. 2021, the fourth paper in the series. We have included a statement to this effect in Sect 2.2 to clarify this.

*Fig. 2: it is hard to distinguish the orange and red crosses.

>>> Reply: We have changed the orange to grey.

*Sect. 3.6, 4th paragraph: It would be really nice to show the AA Tau-like light
curves to convince the readers they are due to circumstellar dust occultation rather
than spots.

>>> Reply: The light curves of the hot spot, cold spot or AA-Tau objects cannot be used to identify them (otherwise it would not be necessary to use our spot fitting method to identify them). Yes, there are some AA-Tau like light curves that allow this, but the ones investigated here can only be identified by the failure to fit any spot model to the multi-wavelength data. The first paragraph of Sect. 3.6 is designed to convince the reader that these objects cannot be differentiated visually from the light curves.

*Sect. 4.1: You say in the text of the manuscript that you analyzed the V, R and I
photometric amplitudes of all the targets, but in Sect. 4 you only discuss the V
amplitudes. What are the results for R and I?

>>> Reply: This seems to be a misunderstanding. Throughout this paper we use a notation that we explain in detail in Sect. 3.2. We refer to the shortest wavelength filter in curly brackets to mean this filter and all longer wavelength filter. In other words: {V} means the set V, R, and I. '{}' being the standard maths notation for 'set'. The results in this section are hence obtained by using V, R, and I amplitudes simultaneously (see also Eq.2). Indeed it would be impossible to determine the spot temperature and size simultaneously from an amplitude measured in a single filter. 

*Sect. 4.1, 1st paragraph: The stars that presented B and U data had their photometric
amplitudes also analyzed in these bands, but you do not list the values in Table 2.
If the analysis was done, why not list the results in the table?

>>> Reply: Yes, the analysis was done for all available filter sets. Note the potential misunderstanding of {U} and {B}, discussed above. However, as discussed in the paper, the signal to noise ratio for amplitudes at these short wavelengths varies significantly in quality, and is generally very low. This is why we list the HS:CS ratio and the SNRs of the B and U amplitudes in Table2. The HS:CS ratio shows whether the spot can be clearly identified as a hot spot or a cold spot, Sect. 4.1, and in particular the 2nd paragraph show that uncertain classification is always coupled to low SNRs for the amplitudes. Given that many sources do not have U and/or B data, and if so their SNR for the amplitudes are generally low, we refrain from including the determined spot properties from the {U} and {B} data in the paper. Our statistical discussion of the results is solely based on the {V} data which is available for all 27 spotted sources. Reliable {B} or {U} data is only available for a very small number of objects (9 and 1 respectively) and thus suffers from small number statistics.

*Sect. 4.1, 2nd paragraph: You say your classification of sources into hot/cold spot
objects was based on the V data because it is available for all objects. But you also
have R and I data for all the objects, so why don't you use all three bands together
to constrain the spots properties?

>>> Reply: Please see our reply about the misunderstanding of {V} and V above.

*Sect. 4.2, 1st paragraph: You say that the hot spot temperatures are lower than what
would be expected for accretion hot spots, and cite Muzerolle et al. (1998) and
Hartmann (1998). Muzerolle et al. (1998) use Teff=4000 K and Tspot= 7200 K,
and Hartmann (1998) is a great book, but finding such a specific information is not
an easy task.

In fact, spot temperatures up to 3000 K above Teff are not significantly cooler than what is typically expected for accretion-driven spots. Actually this is quite normal for hot spots, as can be seen both in observational (Bouvier et al. 1993, 1995) and theoretical (Muzerolle et al. 1998, Kurosawa et al. 2006) works.

>>> Reply: We agree with the referee and have changed the wording of the text in this section, and everywhere else throughout the paper where this was mentioned. 

*Sect. 4.3, 6th paragraph: You would expect that hot spots occur on systems
with infrared excess, but your results point otherwise. How certain are you
of the spot temperature in theses cases? Could they be modeled with cold spots?
Do you have B and U data for those systems?

>>> Reply: The uncertainties for the spot temperatures are listed in Table2, as well as the HS:CS ratios. They show that the cold spot solutions are significantly worse than the hot spot solutions for these sources. In the table one can also see that we only have (low SNR) B data for one of the hot spot objects and no U for any of them.

If TW Hya, which is actively accreting, has K-W2=0.4mag, is it reasonable to use
a threshold of 0.5mag to separate accreting and non-accreting systems? Transition disk systems, with  large inner dust cavities, tend to accrete essentially at the same
level as full disk systems.

>>> Reply: This point is already made in the paper. In the 3rd paragraph of Section 4.3, when we mention the example of TW Hya, we acknowledge that an infrared colour criterion cannot identify (by its nature) all disks. We note that we do not use K-W2 to separate accreting from non-accreting, we use it to separate Class II from Class III. Shifting the threshold to lower K-W2 is not going to help, and would misidentify Class III sources as those with disks. We also explain why we choose 0.5mag as cutoff. No changes have been made to the text. 

What is the expected temperature and coverage for plages? Are they consistent with the hot spot properties that you obtained?

>>> Reply: This is an interesting question. We note that Shapiro et al. 2016 has shown that even for the Sun, light curves can be dominated by hot spots under certain circumstances (viewing angle, timescale). We have added a few notes to clarify this, in order to show that this is a valid potential alternative explanation for hot spots on apparently disk free sources.

*Sect. 5, 3rd paragraph:
Again, I do not agree that spot temperatures up to 3000 K above Teff are significantly
cooler than what is typically expected for accretion-driven spots, as pointed before.

>>> Reply: Agreed, see our reply to the similar point made above.
